A Perturbed-Alexander Invariant

In this note we give concise formulas, which lead to a simple and fast computer program that computes a powerful knot invariant. This invariant $\rho_1$ is not new, yet our formulas are by far the simplest and fastest: given a knot we write one of the standard matrices $A$ whose determinant is its Alexander polynomial, yet instead of computing the determinant we consider a certain quadratic expression in the entries of $A^{-1}$. The proximity of our formulas to the Alexander polynomial suggest that they should have a topological explanation. This we don't have yet.

==> refs4QT.tex <==
\bibitem[BN1]{Talk:Chicago-1009} D.~Bar-Natan,
  From the $ax+b$ Lie Algebra to the Alexander Polynomial and Beyond.
  Talk given at Knots in Chicago, September 2010. Video and handout at \url{http://drorbn.net/Chi10}.

\bibitem[BN2]{Talk:NCSU-1604} D.~Bar-Natan,
  Gauss-Gassner Invariants.
  Talk given at Knots in the Triangle (Knots in Washington XLII), North Carolina State University, April 29
  -- May 1, 2016. Video and handout at \url{http://drorbn.net/NCSU-1604}.

\bibitem[BN3]{Talk:Indiana-1611} D.~Bar-Natan,
  A Poly-Time Knot Polynomial Via Solvable Approximation.
  Talk given at Indiana University, November 7, 2016. Video and handout at
  \url{http://drorbn.net/Indiana-1611}.

\bibitem[BN4]{Talk:LesDiablerets-1708} D.~Bar-Natan,
  The Dogma is Wrong.
  Talk given at Lie Groups in Mathematics and Physics, Les Diablerets, August 2017. Video and handout at
  \url{http://drorbn.net/ld17}.

\bibitem[BN5]{Talk:Toronto-1811} D.~Bar-Natan,
  Computation without Representation.
  Talk given in Toronto, November 21, 2018. Video and handout at
  \url{http://drorbn.net/to18}.

\bibitem[BN6]{Talk:DaNang-1905} D.~Bar-Natan,
  Everything around $\sleps$ is DoPeGDO. So what?
  Talk given at Quantum Topology and Hyperbolic Geometry Conference, Da Nang, Vietnam, May 27--31 2019.
  Video and handout at \url{http://drorbn.net/v19}.

\bibitem[BN7]{Talk:Sydney-190916} D.~Bar-Natan,
  Algebraic Knot Theory.
  Talk given in Sydney, September 16, 2019. Video and handout at \url{http://drorbn.net/syd2}.

\bibitem[BN8]{Talk:UCLA-191101} D.~Bar-Natan,
  Some Feynman Diagrams in Algebra.
  Talk given in UCLA, November 1, 2019. Video and handout at \url{http://drorbn.net/la19}.

\bibitem[BN9]{Talk:Waco-2203} D.~Bar-Natan,
  Cars, Interchanges, Traffic Counters, and a Pretty Darned Good Knot Invariant.
  Talk given at the 55th Spring Topology and Dynamical
  Systems Conference, Waco, March 2022. Video and handout at
  \url{http://drorbn.net/waco22}.

\bibitem[BN10]{Talk:Geneva-2206} D.~Bar-Natan,
  Cars, Interchanges, Traffic Counters, and a Pretty Darned Good Knot Invariant.
  Talk given at ``From Subfactors to Quantum Topology - In memory of Vaughan Jones'',
  Geneva, June 30 2022. Video and handout at
  \url{http://drorbn.net/j22}.

\bibitem[BD]{WKO1} D.~Bar-Natan and Z.~Dancso,
  \href
    {http://drorbn.net/AcademicPensieve/Projects/WKO1}
    {Finite Type Invariants of W-Knotted Objects I: W-Knots and the Alexander Polynomial}.
  \emph{Alg. and Geom. Top.} {\bf 16-2} (2016) 1063--1133,
  \arxiv{1405.1956}.

\bibitem[BNG]{Bar-NatanGaroufalidis:MMR} D.~Bar-Natan and S.~Garoufalidis,
  On the Melvin-Morton-Rozansky conjecture.
  \emph{Invent. Math.} {\bf 125} (1996) 103--133.

\bibitem[BV1]{PP1} D.~Bar-Natan and R.~van~der~Veen,
  A Polynomial Time Knot Polynomial,
  \emph{Proc. Amer. Math. Soc.} {\bf 147} (2019) 377--397, \arxiv{1708.04853}.

\bibitem[BV2]{Talk:Matemale-1804} D.~Bar-Natan and R.~van~der~Veen,
  Talks in Matemale,
  April 2018. Videos and handout at \url{http://drorbn.net/mm18}.

\bibitem[BV3]{PG} D.~Bar-Natan and R.~van~der~Veen,
  Perturbed Gaussian Generating Functions for Universal Knot Invariants.
  2021, \arxiv{2109.02057}.

\bibitem[BV4]{Self} D.~Bar-Natan and R.~van der Veen,
  A Perturbed-Alexander Invariant, (self-reference). Paper and related files at
  \url{http://drorbn.net/APAI}. The published and the \arxiv{2206.12298} editions may be older.

\bibitem[BM]{Bar-NatanMorrison:KnotTheory} D.~Bar-Natan, S.~Morrison, and others,
  {\tt KnotTheory`}, a knot theory mathematica package.
  \url{http://katlas.org/wiki/The_Mathematica_Package_KnotTheory}.

\bibitem[Bu]{Burau:Zopfgruppen} W.~Burau,
  \"Uber Zopfgruppen und gleichsinnig verdrillte Verkettungen.
  \emph{Abh. Math. Semin. Univ. Hamburg} {\bf 11} (1936) 179–-186.

\bibitem[Dr]{Drinfeld:QuantumGroups} V.~G.~Drinfel'd,
  Quantum Groups.
  In \emph{Proc. Int. Cong. Math.}, 798--820, Berkeley, 1986.

\bibitem[ES]{EtingofSchiffman:QuantumGroups} P.~Etingof and O.~Schiffman,
  {\em Lectures on Quantum Groups}.
  International Press, Boston, 1998.

\bibitem[Fo]{Fox:Problems} R.~H.~Fox,
  Some Problems in Knot Theory.
  In \emph{Topology of 3-manifolds and related topics (Proc. The Univ. of Georgia Institute, 1961)},
  pp. 168--176, Prentice-Hall, Englewood Cliffs, N.J.

\bibitem[FM]{FoxMilnor:CobordismOfKnots} R.~H.~Fox and J.~W.~Milnor,
  Singularities of 2-Spheres in 4-Space and Cobordism of Knots.
  \emph{Osaka J. Math.} {\bf 3-2} (1966) 257--267.

\bibitem[GR]{GaroufalidisRozansky:LoopExpansion} S.~Garoufalidis and L.~Rozansky,
  The Loop Expansion of the Kontsevich Integral, the Null Move and $S$-Equivalence.
  \emph{Topology} {\bf 43-5} (2004) 1183--1210, \arxiv{math/0003187}.

\bibitem[GST]{GompfScharlemannThompson:Counterexample} R.~E.~Gompf, M.~Scharlemann, and A.~Thompson,
  Fibered Knots and Potential Counterexamples to the Property 2R and Slice-Ribbon Conjectures.
  \emph{Geom. and Top.} {\bf 14} (2010) 2305--2347, \arxiv{1103.1601}.

\bibitem[Jo]{Jones:Hecke} V.~F.~R.~Jones,
  Hecke Algebra Representations of Braid Groups and Link Polynomials,
  \emph{Annals Math.} {\bf 126} (1987) 335-388.

\bibitem[Kr]{Kricker:Lines} A.~Kricker,
  The Lines of the Kontsevich Integral and Rozansky's Rationality Conjecture.
  \arxiv{math/0005284}.

\bibitem[La1]{Lawrence:UniversalUsingQG} R.~J.~Lawrence,
  Universal Link Invariants using Quantum Groups.
  In \emph{Proc. XVII Int. Conf. on Diff. Geom. Methods in Theor. Phys.}, pp. 55--63, Chester,
  England, August 1988. World Scientific (1989).

\bibitem[La2]{Lawrence:Universal} R.~J.~Lawrence,
  A Universal Link Invariant.
  In \emph{Proc. IMA Conf. Math. --- Particle Phys. Interface,} pp. 151--156, Oxford, England,
  September 1988. Inst. Math. Appl. Conf. Ser. New Ser. {\bf 24},
  Oxford Univ. Press (1990).

\bibitem[LTW]{LinTianWang:RandomWalk} X-S.~Lin, F.~Tian, and Z.~Wang,
  Burau Representation and Random Walk on String Links.
  \emph{Pac. J. Math.} {\bf 182-2} (1998) 289--302, \arxiv{q-alg/9605023}.

\bibitem[MM]{MelvinMorton:Coloured} P.~M.~Melvin and H.~R.~Morton,
  The coloured Jones function.
  \emph{Comm. Math. Phys.} {\bf 169} (1995) 501--520.

\bibitem[Oh]{Ohtsuki:QuantumInvariants} T.~Ohtsuki,
  {\em Quantum Invariants},
  Series on Knots and Everything {\bf 29}, World Scientific 2002.

\bibitem[Ov]{Overbay:Thesis} A.~Overbay,
  {\em Perturbative Expansion of the Colored Jones Polynomial}.
  Ph.D.\ thesis, University of North Carolina, August 2013,
  \url{https://cdr.lib.unc.edu/concern/dissertations/hm50ts889}.

\bibitem[Po]{Polyak:RMoves} M.~Polyak,
  Minimal Generating Sets of Reidemeister Moves.
  \emph{Quantum Topol.} {\bf 1} (2010) 399--411, \arxiv{0908.3127}.

\bibitem[Ro1]{Rozansky:TrivialFlatI} L.~Rozansky,
  A Contribution of the Trivial Flat Connection to the Jones
  Polynomial and Witten's Invariant of 3D Manifolds, I.
  \emph{Comm. Math. Phys.} {\bf 175-2} (1996) 275--296, \arxiv{hep-th/9401061}.

\bibitem[Ro2]{Rozansky:Burau} L.~Rozansky,
  The Universal $R$-Matrix, Burau Representation and the Melvin-Morton
    Expansion of the Colored Jones Polynomial.
  \emph{Adv. Math.} {\bf 134-1} (1998) 1--31, \arxiv{q-alg/9604005}.

\bibitem[Ro3]{Rozansky:U1RCC} L.~Rozansky,
  A Universal $U(1)$-RCC Invariant of Links and Rationality Conjecture.
  2002, \arxiv{math/0201139}.

\bibitem[Sch]{Schaveling:Thesis} S.~Schaveling,
  {\em Expansions of Quantum Group Invariants}.
  Ph.D. thesis, Universiteit Leiden, September 2020,
  \url{https://scholarlypublications.universiteitleiden.nl/handle/1887/136272}.

\bibitem[St]{Storjohann:ComplexityOfInversion} A.~Storjohann,
  On the Complexity of Inverting Integer and Polynomial Matrices.
  \emph{Comput. Complex.} {\bf 24} (2015) 777-–821.

\bibitem[Wo]{Wolfram:Mathematica}
  Wolfram Language \& System Documentation Center.
  \url{https://reference.wolfram.com/language/}.

